Distributed and Asynchronous Operational Optimization of Networked Microgrids

Smart programmable microgrids (SPM) is an emerging technology for making microgrids more software-defined and less hardware-independent such that converting distributed energy resources (DERs) to networked community microgrids becomes affordable, autonomic, and secure. As one of the cornerstones of SPM, this paper pioneers a concept of software-defined operation optimization for networked microgrids, where operation objectives, grid connection, and DER participation will be defined by software and plug-and-play, and can be quickly reconfigured, based on the development of modularized and tightened models and a novel asynchronous price-based decomposition-and-coordination method. Key contributions include: (1) design the architecture of the operational optimization of networked microgrids which can be readily implemented to ensure the programmability of islanded microgrids in solving the distributed optimization models, (2) realize a novel discrete model of droop controller, and (3) introduce a powerful distributed and asynchronous method Distributed and Asynchronous Surrogate Lagrangian Relaxation (DA-SLR) to efficiently coordinate microgrids asynchronously. Two case studies are tested to demonstrate the efficiency of developed DA-SLR, and specifically, the testing results show the superiority of DA-SLR as compared to previous methods such as ADMM.

==> NMGsStructure.tex <==
\section{General description of the proposed model}\label{section:02}
In the designed model, a networked structure of islanded microgrids is considered. Each microgrid is connected to one or a group of neighbour MGs. Therefore, the control center of MGs should collect data from their local controllers to make an accurate decision about the power exchanging possibility with neighbour MGs. All autonomous MGs consist of dispatchable and nondispatchable generators and loads. In this structure, MG control center observes the difference between generation and load, and then decides about power exchange with other MGs. In the presented structure, each MG is considered as an autonomous entity. To guarantee the operational optimization of networked MGs, the correlation between all MG entities should be optimally coordinated. In this paper, a distributed algorithm is employed to satisfy the coordination between entities. In Fig. \ref{fig01}, a general description for optimal connection between islanded MGs can be seen.
\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.40\textwidth]{images/01-architecture.png}
\caption{\small Networked MG-based distribution grid }
\label{fig01}%\vspace{-10px}
\end{figure}

The distributed optimization model of the proposed framework in Fig. \ref{fig01} is discussed in the next section.


==> Nomenclature.tex <==
%\section{Nomenclature}\label{sez:4\part{title}}
\vspace{-5px}
%\vspace{8px}
	\mbox{}
	%\scriptsize{
%		\footnotesize {
	\setlength{\nomlabelwidth}{2cm}
	\setlength{\nomitemsep}{-\parsep}
	    \nomenclature[A,01]{$t$}{Index of time}
	    \nomenclature[A,02]{$r$}{Index for iteration number of DA-SLR}
	    \nomenclature[A,03]{$m, w$}{Indices of microgrids}
	    \nomenclature[A,04]{$c$}{Index of battery}
	    \nomenclature[A,05]{$n,k$}{Indices of bus}
	    
	    
		\nomenclature[B,01]{$\alpha^{g}$}{Power generation price of dispatchable DGs}
		\nomenclature[B,02]{$\alpha_{ch}^{BAT}$}{Charging price of the battery}
		\nomenclature[B,03]{$\alpha_{dch}^{BAT}$}{Discharging price of the battery}
		\nomenclature[B,04]{$f_{ref}$}{Nominal frequency [Hz]}
		\nomenclature[B,05]{$V_{ref}$}{Nominal voltage magnitude [v]}
		\nomenclature[B,06]{$V_{0}$}{The bus voltage magnitude of point of common coupling in an MG [v]}
		\nomenclature[B,07]{$r_{n,k}$}{Distribution line resistance between nodes $n$ and $k$}
		\nomenclature[B,08]{$x_{n,k}$}{Distribution line reactance between nodes $n$ and $k$}
		\nomenclature[B,09]{$\zeta_{IL}$}{Interrupted power price}
		\nomenclature[B,10]{$s_{n}^{g}$}{Connection indicator of a generator to node $n$}
		\nomenclature[B,11]{$s_{n}^{BAT}$}{Connection indicator of a battery to node $n$}
		\nomenclature[B,12]{$s_{n-m}^{Tran}$}{Connection indicator of node $n$ to a node in neighbour MG $m$}
		\nomenclature[B,13]{$P_{t}^{g,WT}$}{Real power generation of a wind turbine at time $t$ [kW]}
		\nomenclature[B,14]{$P_{t}^{g,PV}$}{Real power generation of a PV at time $t$ [kW]}
		\nomenclature[B,15]{$Q_{t}^{g,WT}$}{Reactive power generation of a wind turbine at time $t$ [kvar]}
		\nomenclature[B,16]{$Q_{t}^{g,PV}$}{Reactive power generation of a PV at time $t$ [kvar]}
		
		\nomenclature[c,01]{$P^{g,MT}$}{Generated power by MT [kW]}
		\nomenclature[c,02]{$P^{g,FC}$}{Generated power by FC [kW]}
		\nomenclature[c,03]{$P^{g,CHP}$}{Generated power by CHP [kW]}
		\nomenclature[c,04]{$P^{BAT,ch}$}{Charging power of battery [kW]}
		\nomenclature[c,05]{$P^{BAT,dch}$}{Discharging power of battery [kW]}
		\nomenclature[c,06]{$Q^{g,DG}$}{Generated reactive power of a DG [kW]}
		\nomenclature[c,07]{$f$}{Frequency [Hz]}
		\nomenclature[c,08]{$V$}{Voltage magnitude [v]}
		\nomenclature[c,09]{$m_{p}$}{f-P related droop coefficient}
		\nomenclature[c,10]{$m_{q}$}{V-Q related droop coefficient}
		\nomenclature[c,11]{$P_{(t,n-k)}^{flow}$}{Real power flow between nodes $n$ and $k$ at hour $t$}
		\nomenclature[c,12]{$Q_{(t,n-k)}^{flow}$}{Reactive power flow between nodes $n$ and $k$ at hour $t$}
		\nomenclature[c,13]{$P_{(t,k)}^{L}$}{Real load power in node $k$ at hour $t$}
		\nomenclature[c,14]{$Q_{(t,k)}^{L}$}{Reactive load power in node $k$ at hour $t$}
		\nomenclature[c,15]{$C_{g}$}{Power generation cost [\$/kWh]}
		\nomenclature[c,16]{$C_{ch}$}{Battery charging cost [\$/kWh]}
		\nomenclature[c,17]{$C_{dch}$}{Battery discharging cost [\$/kWh]}
		\nomenclature[c,18]{$P^{IL}$}{Real power interruption [kW]}
		\nomenclature[c,19]{$Q^{IL}$}{Reactive power interruption [kvar]}
		\nomenclature[c,20]{$u^{g}$}{Commitment status of a generator}
		\nomenclature[c,21]{$u^{buy}$}{Status of purchasing power buy MG $m$}
		\nomenclature[c,22]{$P_{(t,m)}^{buy}$}{Real purchased power by MG $m$ at hour $t$ [kW]}
		\nomenclature[c,23]{$P_{(t,m)}^{sell}$}{Real sold power by MG $m$ at hour $t$ [kW]}
		\nomenclature[c,24]{$Q_{(t,m)}^{buy}$}{Reactive purchased power by MG $m$ at hour $t$ [kvar]}
		\nomenclature[c,25]{$Q_{(t,m)}^{sell}$}{Reactive sold power by MG $m$ at hour $t$ [kvar]}
		\nomenclature[c,26]{$u^{ch}$}{Status of charging power by a battery}
		\nomenclature[c,27]{$\lambda^{\alpha}$}{$\alpha th$ Lagrange multiplier}
		
		
		\nomenclature[D,01]{$MG$}{Microgrid}
		\nomenclature[D,02]{$DER$}{Distributed energy resource}
		\nomenclature[D,03]{$DNO$}{Distribution network operator}
		\nomenclature[D,04]{$WT$}{Wind turbine}
		\nomenclature[D,05]{$PV$}{Photovoltaic panel}
		
	
	\printnomenclature
%}\vspace{-5px} 

==> extra.tex <==
\begin{equation}
\label{eq02}\footnotesize
\begin{split}
Cost_{tran,DN}=\sum_{t\in T}[(\lambda_{DN-ws}^{buy,t}\times P_{DN-ws}^{buy,t}-\lambda_{DN-ws}^{sell,t}\times P_{DN-ws}^{sell,t})+\\
(\lambda_{DN-MG}^{buy,t}\times P_{DN-MG}^{buy,t}-\lambda_{DN-MG}^{sell,t}\times P_{DN-MG}^{sell,t})],\quad\forall t\in T
\end{split}
\end{equation}
\begin{equation}
\label{eq03}\footnotesize
\begin{split}
Cost_{batt,DN}=\sum_{t\in T}(\lambda_{ch,DN}^{t}\times P_{ch,DN}^{t}-\lambda_{dch,DN}^{t}\times P_{dch,DN}^{t}),\quad\forall t\in T
\end{split}
\end{equation}
\begin{equation}
\label{eq04}\footnotesize
\begin{split}
Cost_{int,DN}=\sum_{t\in T}(\lambda_{int,DN}^{t}\times P_{int,DN}^{t}),\quad\forall t\in T
\end{split}
\end{equation}
\begin{equation}
\label{eq05}\footnotesize
\begin{split}
Cost_{g,DN}=\sum_{t\in T}(C_{g,MT}^{DN,t}+C_{g,FC}^{DN,t}+C_{g,CHP}^{DN,t}+C_{g,DS}^{DN,t}),\quad\forall t\in T
\end{split}
\end{equation}
\begin{equation}
\label{eq06}\footnotesize
\begin{split}
C_{g,MT}^{DN}=\sum_{mt\in MT}(\frac{C_{nl}}{L}\times \frac{P_{g,mt}}{\eta_{MT}} ),\quad\forall mt\in MT
\end{split}
\end{equation}
\begin{equation}
\label{eq07}\footnotesize
\begin{split}
C_{g,FC}^{DN}=\sum_{fc\in FC}(\frac{C_{nl}}{L}\times \frac{P_{g,fc}}{\eta_{FC}} ),\quad\forall fc\in FC
\end{split}
\end{equation}
\begin{equation}
\label{eq08}\footnotesize
\begin{split}
C_{g,CHP}^{DN}=\sum_{c\in C}(C_{g,MT}^{DN}\times (1-\frac{\epsilon_{rec}\times (\eta_{CHP}-\eta_{MT})}{\eta_{b}}) ),\quad\forall c\in C
\end{split}
\end{equation}
\begin{equation}
\label{eq09}\footnotesize
\begin{split}
C_{g,DS}^{DN}=\sum_{d\in D}(\alpha (P_{g,d})^2+\beta (P_{g,d})+\gamma),\quad\forall d\in D
\end{split}
\end{equation}

In aforementioned equations, the cost dealing with electricity transactions is mentioned in (\ref{eq02}), in which
distribution network can exchange electricity with wholesale market and microgrids. The purchasing power
increases the economic costs of the entity, while distribution network can get profit through selling surplus
electricity to the MGs and wholesale market. Similarly, battery bank cost comprises the charging and
discharging costs in (\ref{eq03}). The interruption cost is described in (\ref{eq04}). The generation or fuel cost of various units is
formulated as (\ref{eq05}). In this regard, the generation costs of microturbine (MT), fuel cell (FC), CHP, and diesel
generator are described as (\ref{eq06}), (\ref{eq07}), (\ref{eq08}), and (\ref{eq09}), respectively.
\subsection{Multi-microgrids}\label{Subsection:02:02}
Similar to distribution network, MGs can address the electricity demand using local energy sources,
energy storage systems, and energy interaction with upper-level supplier. Microgrids and distribution
network are operating in decentralized mode meaning that each sub-system optimizes its objective function
without interference of other entity. So, this operation mode greatly helps the entities to protect the
important data and information and guarantee the security issues. Likewise the distribution network, MGs
have to address the electricity loads at any time slot. Therefore, the objective function of each
MG can be written as follows:
\begin{equation}
\label{eq10}\footnotesize
\begin{split}
Min\ OF^{MG}=\sum_{t\in T}(Cost_{g,MG}^t+Cost_{tran,MG}^t+\\
Cost_{batt,MG}^t+Cost_{int,MG}^t),\quad\forall t\in T
\end{split}
\end{equation}

The costs dealing with electricity transaction, electrical energy storage, and interruption are formulated like DN (\ref{eq02}-\ref{eq04}). However, in case of transacted electrical power of each MG, it should be noted that each MG has only energy interaction with DN. Therefore, the electrical power transaction of each MG can be defined as below:
\begin{equation}
\label{eq11}\footnotesize
\begin{split}
Cost_{tran,MG}=\sum_{t\in T}(\lambda_{DN-MG}^{buy,t}\times P_{DN-MG}^{buy,t}-\lambda_{DN-MG}^{sell,t}\times P_{DN-MG}^{sell,t}),\\ \quad\forall t\in T
\end{split}
\end{equation}



For DN, the active and reactive power balance constraints at bus m at hour t could be written as follow for PQ buses:
\begin{equation}
\label{eq21}\footnotesize
\begin{split}
PL_{m}^{DN,t}-P_{DN-ws}^t-\sum_{mg \in (MG)}(P_{tran}^{DN-MG,t})-(P_{dch}^{DN,t}-P_{ch}^{DN,t})=\\ 
P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, m,n\in M, mg\in MG
\end{split}
\end{equation}
\begin{equation}
\label{eq22}\footnotesize
\begin{split}
QL_{m}^{DN,t}-Q_{DN-ws}^t=\\ 
Q_{nm}^{flow,t}-x_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(Q_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}



\begin{equation}
\label{e01}\footnotesize
\begin{cases}
      P_{mg=1,t}^{buy,MG1-MG2}=P_{mg=2,t}^{sell,MG2-MG1} \\
      P_{mg=1,t}^{buy,MG1-MG3}=P_{mg=3,t}^{sell,MG3-MG1} \\
      P_{mg=2,t}^{buy,MG2-MG3}=P_{mg=3,t}^{sell,MG3-MG2} \\
      P_{mg=2,t}^{buy,MG2-MG1}=P_{mg=1,t}^{sell,MG1-MG2} \\
      P_{mg=3,t}^{buy,MG3-MG1}=P_{mg=1,t}^{sell,MG1-MG3} \\
      P_{mg=3,t}^{buy,MG3-MG2}=P_{mg=2,t}^{sell,MG2-MG3}
\end{cases}
\end{equation}



After relaxing the constraints (\ref{e01}) by defining 6 multipliers, the Lagrangian function becomes:
\begin{equation}
\label{e02}\footnotesize
\begin{split}
L(P,\lambda)=\sum_{mg \in MG}[\sum_{g\in DG}(c_{(t=1,mg,g)}^G\times P_{(t=1,mg,g)}^G)\\
+\sum_{mg \in MG}[\sum_{c\in BAT}(c_{(t=1,mg,c)}^{ch}\times P_{(t=1,mg,c)}^{ch}-c_{(t=1,mg,c)}^{dch}\times P_{(t=1,mg,c)}^{dch})\\
+\lambda_{1}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG2}-P_{mg=2,t}^{sell,MG2-MG1})\\
+\lambda_{2}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG3}-P_{mg=3,t}^{sell,MG3-MG1})\\
+\lambda_{3}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG3}-P_{mg=3,t}^{sell,MG3-MG2}) \\
+\lambda_{4}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG1}-P_{mg=1,t}^{sell,MG1-MG2})\\
+\lambda_{5}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG1}-P_{mg=1,t}^{sell,MG1-MG3})\\
+\lambda_{6}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG2}-P_{mg=2,t}^{sell,MG2-MG3})
\end{split}
\end{equation}




Given the objective function, and coupling constraints, the relaxed problem can be separated into sub-problems as follows:
\begin{equation}
\label{e03}\footnotesize
\begin{split}
\underset{mg=MG1}{min}\{\sum_{g\in DG}(c_{(t=1,mg=1,g)}^G\times P_{(t=1,mg=1,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=1,c)}^{ch}\times P_{(t=1,mg=1,c)}^{ch}\\
-c_{(t=1,mg=1,c)}^{dch}\times P_{(t=1,mg=1,c)}^{dch})]\\
+\lambda_{1}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG2})+\lambda_{2}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG3})\\
-\lambda_{4}^{(t=1)}(P_{mg=1,t}^{sell,MG1-MG2})-\lambda_{5}^{(t=1)}(P_{mg=1,t}^{sell,MG1-MG3})\}
\end{split}
\end{equation}\\

\begin{equation}
\label{e04}\footnotesize
\begin{split}
\underset{mg=MG2}{min}\{\sum_{g\in DG}(c_{(t=1,mg=2,g)}^G\times P_{(t=1,mg=2,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=2,c)}^{ch}\times P_{(t=1,mg=2,c)}^{ch}\\
-c_{(t=1,mg=2,c)}^{dch}\times P_{(t=1,mg=2,c)}^{dch})]\\
+\lambda_{3}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG3})+\lambda_{4}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG1})\\
-\lambda_{1}^{(t=1)}(P_{mg=2,t}^{sell,MG2-MG1})-\lambda_{6}^{(t=1)}(P_{mg=2,t}^{sell,MG2-MG3})\}
\end{split}
\end{equation}\\

\begin{equation}
\label{e05}\footnotesize
\begin{split}
\underset{mg=MG3}{min}\{\sum_{g\in DG}(c_{(t=1,mg=3,g)}^G\times P_{(t=1,mg=3,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=3,c)}^{ch}\times P_{(t=1,mg=3,c)}^{ch}\\
-c_{(t=1,mg=3,c)}^{dch}\times P_{(t=1,mg=3,c)}^{dch})]\\
+\lambda_{5}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG1})+\lambda_{6}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG2})\\
-\lambda_{2}^{(t=1)}(P_{mg=3,t}^{sell,MG3-MG1})-\lambda_{3}^{(t=1)}(P_{mg=3,t}^{sell,MG3-MG2})\}
\end{split}
\end{equation}





\begin{equation}
\label{e03}\footnotesize
\begin{split}
\underset{mg=MG1}{min}\{\sum_{g\in DG}(c_{(t=1,mg=1,g)}^G\times P_{(t=1,mg=1,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=1,c)}^{ch}\times P_{(t=1,mg=1,c)}^{ch}\\
-c_{(t=1,mg=1,c)}^{dch}\times P_{(t=1,mg=1,c)}^{dch})]\\
+\lambda_{1}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG2})+\lambda_{2}^{(t=1)}(P_{mg=1,t}^{buy,MG1-MG3})\\
-\lambda_{4}^{(t=1)}(P_{mg=1,t}^{sell,MG1-MG2})-\lambda_{5}^{(t=1)}(P_{mg=1,t}^{sell,MG1-MG3})\}
\end{split}
\end{equation}\\

\begin{equation}
\label{e04}\footnotesize
\begin{split}
\underset{mg=MG2}{min}\{\sum_{g\in DG}(c_{(t=1,mg=2,g)}^G\times P_{(t=1,mg=2,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=2,c)}^{ch}\times P_{(t=1,mg=2,c)}^{ch}\\
-c_{(t=1,mg=2,c)}^{dch}\times P_{(t=1,mg=2,c)}^{dch})]\\
+\lambda_{3}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG3})+\lambda_{4}^{(t=1)}(P_{mg=2,t}^{buy,MG2-MG1})\\
-\lambda_{1}^{(t=1)}(P_{mg=2,t}^{sell,MG2-MG1})-\lambda_{6}^{(t=1)}(P_{mg=2,t}^{sell,MG2-MG3})\}
\end{split}
\end{equation}\\

\begin{equation}
\label{e05}\footnotesize
\begin{split}
\underset{mg=MG3}{min}\{\sum_{g\in DG}(c_{(t=1,mg=3,g)}^G\times P_{(t=1,mg=3,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t=1,mg=3,c)}^{ch}\times P_{(t=1,mg=3,c)}^{ch}\\
-c_{(t=1,mg=3,c)}^{dch}\times P_{(t=1,mg=3,c)}^{dch})]\\
+\lambda_{5}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG1})+\lambda_{6}^{(t=1)}(P_{mg=3,t}^{buy,MG3-MG2})\\
-\lambda_{2}^{(t=1)}(P_{mg=3,t}^{sell,MG3-MG1})-\lambda_{3}^{(t=1)}(P_{mg=3,t}^{sell,MG3-MG2})\}
\end{split}
\end{equation}





1) The coordinator initializes $(P_{mg=1,t}^{buy,MG1-MG2})^{j=0}$, $(P_{mg=1,t}^{buy,MG1-MG3})^{j=0}$, $(P_{mg=2,t}^{buy,MG2-MG3})^{j=0}$, $(P_{mg=2,t}^{buy,MG2-MG1})^{j=0}$, $(P_{mg=3,t}^{buy,MG3-MG1})^{j=0}$, $(P_{mg=3,t}^{buy,MG3-MG2})^{j=0}$, $(P_{mg=2,t}^{sell,MG2-MG1})^{j=0}$, $(P_{mg=3,t}^{sell,MG3-MG1})^{j=0}$, $(P_{mg=3,t}^{sell,MG3-MG2})^{j=0}$, $(P_{mg=1,t}^{sell,MG1-MG2})^{j=0}$, $(P_{mg=1,t}^{sell,MG1-MG3})^{j=0}$, and $(P_{mg=2,t}^{sell,MG2-MG3})^{j=0}$.





\begin{equation}
\label{r04}\footnotesize
\begin{bmatrix}
(\lambda_{1}^{t})^{j+1}\\
(\lambda_{2}^{t})^{j+1}\\
\vdots \\
(\lambda_{m(m-1)}^{t})^{j+1}
\end{bmatrix}
=
\begin{bmatrix}
(\lambda_{1}^{t})^{j}\\
(\lambda_{2}^{t})^{j}\\
\vdots \\
(\lambda_{m(m-1)}^{t})^{j}
\end{bmatrix}
+s^{j}
\begin{bmatrix}
    (P_{mg=1,t}^{buy,MG1-MG2})^{j}-(P_{mg=2,t}^{sell,MG2-MG1})^{j} \\
    (P_{mg=1,t}^{buy,MG1-MG3})^{j}-(P_{mg=3,t}^{sell,MG3-MG1})^{j} \\
    \vdots \\
    (P_{mg=m,t}^{buy,MGm-MGn})^{j}-(P_{mg=n,t}^{sell,MGn-MGm})^{j}
\end{bmatrix}



      (\lambda_{1}^{t})^{j+1}=(\lambda_{1}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG2})^{j+1}-(P_{mg=2,t}^{sell,MG2-MG1})^{j}) \\
      (\lambda_{2}^{t})^{j+1}=(\lambda_{2}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG3})^{j+1}-(P_{mg=3,t}^{sell,MG3-MG1})^{j}) \\
      (\lambda_{3}^{t})^{j+1}=(\lambda_{3}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG3})^{j}-(P_{mg=3,t}^{sell,MG3-MG2})^{j}) \\
      (\lambda_{4}^{t})^{j+1}=(\lambda_{4}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG1})^{j}-(P_{mg=1,t}^{sell,MG1-MG2})^{j+1}) \\
      (\lambda_{5}^{t})^{j+1}=(\lambda_{5}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG1})^{j}-(P_{mg=1,t}^{sell,MG1-MG3})^{j+1}) \\
      (\lambda_{6}^{t})^{j+1}=(\lambda_{6}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG2})^{j}-(P_{mg=2,t}^{sell,MG2-MG3})^{j})
\end{equation}





To have a better understanding, take the network with 3 MGs as an example. After sending the initial values of $\lambda$ by the coordinator to all MGs, all 3 MGs optimize their objective function. Then, MG1 sends its updated purchased and sold powers amounts e.g., $(P_{mg=1,t}^{buy,MG1-MG2})^{j+1}$, $(P_{mg=1,t}^{buy,MG1-MG3})^{j+1}$, $(P_{mg=1,t}^{sell,MG1-MG2})^{j+1}$, and $(P_{mg=1,t}^{sell,MG1-MG3})^{j+1}$ to the coordinator. Now, the coordinator will use the following purchased and sold powers to update multipliers:\\
$(P_{mg=1,t}^{buy,MG1-MG2})^{j+1}$, $(P_{mg=1,t}^{buy,MG1-MG3})^{j+1}$, $(P_{mg=2,t}^{buy,MG2-MG3})^{j}$, $(P_{mg=2,t}^{buy,MG2-MG1})^{j}$, $(P_{mg=3,t}^{buy,MG3-MG1})^{j}$, $(P_{mg=3,t}^{buy,MG3-MG2})^{j}$, $(P_{mg=2,t}^{sell,MG2-MG1})^{j}$, $(P_{mg=3,t}^{sell,MG3-MG1})^{j}$, $(P_{mg=3,t}^{sell,MG3-MG2})^{j}$, $(P_{mg=1,t}^{sell,MG1-MG2})^{j+1}$, $(P_{mg=1,t}^{sell,MG1-MG3})^{j+1}$, and $(P_{mg=2,t}^{sell,MG2-MG3})^{j}$.

Therefore, the updated multipliers by coordinator will be as follows:
\begin{equation}
\label{e06}\footnotesize
\begin{cases}
      (\lambda_{1}^{t})^{j+1}=(\lambda_{1}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG2})^{j+1}-(P_{mg=2,t}^{sell,MG2-MG1})^{j}) \\
      (\lambda_{2}^{t})^{j+1}=(\lambda_{2}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG3})^{j+1}-(P_{mg=3,t}^{sell,MG3-MG1})^{j}) \\
      (\lambda_{3}^{t})^{j+1}=(\lambda_{3}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG3})^{j}-(P_{mg=3,t}^{sell,MG3-MG2})^{j}) \\
      (\lambda_{4}^{t})^{j+1}=(\lambda_{4}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG1})^{j}-(P_{mg=1,t}^{sell,MG1-MG2})^{j+1}) \\
      (\lambda_{5}^{t})^{j+1}=(\lambda_{5}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG1})^{j}-(P_{mg=1,t}^{sell,MG1-MG3})^{j+1}) \\
      (\lambda_{6}^{t})^{j+1}=(\lambda_{6}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG2})^{j}-(P_{mg=2,t}^{sell,MG2-MG3})^{j})
\end{cases}
\end{equation}








As we can see, only $\lambda_{1}^{t}$, $\lambda_{2}^{t}$, $\lambda_{4}^{t}$ and $\lambda_{5}^{t}$ are updated and sent to all MGs. If the surrogate optimality condition for sub-problems is not satisfied, then we should go to the next step to update other multipliers as well.

3) In this step, firstly, all sub-problems are optimized based on the new $\lambda_{1}^{t}$, $\lambda_{2}^{t}$, $\lambda_{4}^{t}$ and $\lambda_{5}^{t}$. MG2 sends its updated purchased and sold powers to the coordinator e.g., $(P_{mg=2,t}^{buy,MG2-MG1})$, $(P_{mg=2,t}^{buy,MG2-MG3})$, $(P_{mg=2,t}^{sell,MG2-MG1})$, and $(P_{mg=2,t}^{sell,MG2-MG3})$, so that the coordinator updates all possible multipliers. Now, the coordinator will use the following purchased and sold powers to update multipliers:
$(P_{mg=1,t}^{buy,MG1-MG2})^{j}$, $(P_{mg=1,t}^{buy,MG1-MG3})^{j}$, $(P_{mg=2,t}^{buy,MG2-MG3})^{j+1}$, $(P_{mg=2,t}^{buy,MG2-MG1})^{j+1}$, $(P_{mg=3,t}^{buy,MG3-MG1})^{j-1}$, $(P_{mg=3,t}^{buy,MG3-MG2})^{j-1}$, $(P_{mg=2,t}^{sell,MG2-MG1})^{j+1}$, $(P_{mg=3,t}^{sell,MG3-MG1})^{j-1}$, $(P_{mg=3,t}^{sell,MG3-MG2})^{j-1}$, $(P_{mg=1,t}^{sell,MG1-MG2})^{j}$, $(P_{mg=1,t}^{sell,MG1-MG3})^{j}$, and $(P_{mg=2,t}^{sell,MG2-MG3})^{j+1}$.

So, we can see that the coordinator will use the new power amounts of MG2, the power amounts of MG1 in previous step, and the initialized power values of MG3 in the first step. Therefore, the updated multipliers by coordinator will be as follows:
\begin{equation}
\label{e07}\footnotesize
\begin{cases}
      (\lambda_{1}^{t})^{j+1}=(\lambda_{1}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG2})^{j}-(P_{mg=2,t}^{sell,MG2-MG1})^{j+1}) \\
      (\lambda_{2}^{t})^{j+1}=(\lambda_{2}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG3})^{j}-(P_{mg=3,t}^{sell,MG3-MG1})^{j-1}) \\
      (\lambda_{3}^{t})^{j+1}=(\lambda_{3}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG3})^{j+1}-(P_{mg=3,t}^{sell,MG3-MG2})^{j-1}) \\
      (\lambda_{4}^{t})^{j+1}=(\lambda_{4}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG1})^{j+1}-(P_{mg=1,t}^{sell,MG1-MG2})^{j}) \\
      (\lambda_{5}^{t})^{j+1}=(\lambda_{5}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG1})^{j-1}-(P_{mg=1,t}^{sell,MG1-MG3})^{j}) \\
      (\lambda_{6}^{t})^{j+1}=(\lambda_{6}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG2})^{j-1}-(P_{mg=2,t}^{sell,MG2-MG3})^{j+1})
\end{cases}
\end{equation}

As we can see, only $\lambda_{1}^{t}$, $\lambda_{3}^{t}$, $\lambda_{4}^{t}$ and $\lambda_{6}^{t}$ are updated and sent to all MGs. If the surrogate optimality condition for sub-problems is not satisfied, then we should go to the next step to update other multipliers as well.

4) In this step, firstly, all sub-problems are optimized based on the newly updated multipliers. MG3 sends its updated purchased and sold powers to the coordinator e.g., $(P_{mg=3,t}^{buy,MG3-MG1})$, $(P_{mg=3,t}^{buy,MG3-MG2})$, $(P_{mg=3,t}^{sell,MG3-MG1})$, and $(P_{mg=3,t}^{sell,MG3-MG2})$, so that the coordinator updates all possible multipliers. So, we can see that the coordinator will use the new power amounts of MG3, the power amounts of MG2 in previous step, and the power values of MG1 in two iteration before this step. Therefore, the updated multipliers by coordinator will be as follows:
\begin{equation}
\label{e08}\footnotesize
\begin{cases}
      (\lambda_{1}^{t})^{j+1}=(\lambda_{1}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG2})^{j-1}-(P_{mg=2,t}^{sell,MG2-MG1})^{j}) \\
      (\lambda_{2}^{t})^{j+1}=(\lambda_{2}^{t})^{j}+\pho ((P_{mg=1,t}^{buy,MG1-MG3})^{j-1}-(P_{mg=3,t}^{sell,MG3-MG1})^{j+1}) \\
      (\lambda_{3}^{t})^{j+1}=(\lambda_{3}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG3})^{j}-(P_{mg=3,t}^{sell,MG3-MG2})^{j+1}) \\
      (\lambda_{4}^{t})^{j+1}=(\lambda_{4}^{t})^{j}+\pho ((P_{mg=2,t}^{buy,MG2-MG1})^{j}-(P_{mg=1,t}^{sell,MG1-MG2})^{j-1}) \\
      (\lambda_{5}^{t})^{j+1}=(\lambda_{5}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG1})^{j+1}-(P_{mg=1,t}^{sell,MG1-MG3})^{j-1}) \\
      (\lambda_{6}^{t})^{j+1}=(\lambda_{6}^{t})^{j}+\pho ((P_{mg=3,t}^{buy,MG3-MG2})^{j+1}-(P_{mg=2,t}^{sell,MG2-MG3})^{j})
\end{cases}
\end{equation}

As we can see, only $\lambda_{2}^{t}$, $\lambda_{3}^{t}$, $\lambda_{5}^{t}$ and $\lambda_{6}^{t}$ are updated and sent to all MGs. If the surrogate optimality condition for sub-problems is not satisfied, then we should go to the next step to update other multipliers as well.

5)	This procedure continues till the surrogate optimality condition for sub-problems is satisfied.





The complex power flow equations associated with bus m can be described as follows:
\begin{equation}
\label{eq17}\footnotesize
\begin{split}
PL_{m}^t=P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}), \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}
\begin{equation}
\label{eq18}\footnotesize
\begin{split}
QL_{m}^t=Q_{nm}^{flow,t}-x_{nm}\times l_{nm}^t-\sum_{\kappa \in (m,\kappa)}(Q_{m\kappa}^{flow,t}), \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}
\begin{equation}
\label{eq19}\footnotesize
\begin{split}
v_{m}^t=v_{n}^t-2(r_{nm}\times P_{nm}^{flow,t}+x_{nm}\times Q_{nm}^{flow,t})+(r_{nm}^2+x_{nm}^2)\times l_{nm}^t,\\
\quad\forall t\in T, m,n\in M
\end{split}
\end{equation}
\begin{equation}
\label{eq20}\footnotesize
\begin{split}
l_{nm}^t=\frac{(P_{nm}^{flow,t})^2+(Q_{nm}^{flow,t})^2}{v_{m}^t},\quad\forall t\in T, m,n\in M
\end{split}
\end{equation}

where $l_{mn}=|I_{mn}|^2$, and $v_{m}=|V_{m}|^2$.








\begin{equation}
\label{eq25}\footnotesize
\begin{split}
PL^{m}_{mg,t}-P^{G,WT}_{mg,t}-P^{G,PV}_{mg,t}-(P^{buy}_{mg,t}-P^{sell}_{mg,t})-\\
(P^{dch}_{mg,t}-P^{ch}_{mg,t})=P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}
\begin{equation}
\label{eq26}\footnotesize
\begin{split}
QL^{m}_{mg,t}-Q^{G,WT}_{mg,t}-Q^{G,PV}_{mg,t}=\\
Q_{nm}^{flow,t}-x_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(Q_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}






\begin{equation}
\label{eq033}\footnotesize
\begin{split}
PL^{m}_{mg,t}-\frac{1}{m_{p}}(f^{ref}_{mg,t}-f_{mg,t})-(P^{buy}_{mg,t}-P^{sell}_{mg,t})-\\
(P^{dch}_{mg,t}-P^{ch}_{mg,t})=P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, m,n\in M
\end{split}
\end{equation}
\begin{equation}
\label{eq034}\footnotesize
\begin{split}
QL^{m}_{mg,t}-\frac{1}{m_{p}}(|V|^{ref,m}_{MG,t}-|V|^{m}_{mg,t})=\\
Q_{nm}^{flow,t}-x_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(Q_{m\kappa}^{flow,t}),\\ \quad\forall t\in T
\end{split}
\end{equation}




\begin{align}
\label{r02}%\footnotesize
\begin{split}
& L(P,\lambda)=\sum_{mg \in MG}[\sum_{g\in DG}(c_{(t,mg,g)}^G\times P_{(t,mg,g)}^G)\\
& +\sum_{mg \in MG}[\sum_{c\in BAT}(c_{(t,mg,c)}^{ch}\times P_{(t,mg,c)}^{ch}-c_{(t,mg,c)}^{dch}\times P_{(t,mg,c)}^{dch})\\
& +[\lambda_{1}^{t} \ \lambda_{2}^{t} \dots \lambda_{TC}^{t}].[P_{MGm,t}^{buy,MGm-MGn}-P_{MGn,t}^{sell,MGn-MGm}]_{TC\times 1} ,\ \quad \forall t\in T,\ m\in M
\end{split}
\end{align}





Consider the following constraints:
Assume we have m/n number of islanding MGs. The purchased power by MG-m from MG-n is equal to the sold power by MG-n to MG-m.
\begin{equation}
\label{r01}\footnotesize
P_{t}^{buy,MGm-MGn}=P_{t}^{sell,MGn-MGm}, \quad\forall t\in T, m,n\in M
\end{equation}

According to (\ref{r01}), increasing the number of MGs causes increasing in the number of constraints. If we have $m$ number of MG, the total number of constraints in (\ref{r01}) will be $m(m-1)$, which means that $m$ number of MGs can connect to the rest of $m-1$ MGs to provide their requirements.

After relaxing the $m(m-1)$ constraints in a network with $m$ MGs, we should define $m(m-1)$ multipliers to establish the Lagrangian function as follows:
\begin{equation}
\label{r02}\footnotesize
\begin{split}
L(P,\lambda)=\sum_{mg \in MG}[\sum_{g\in DG}(c_{(t=1,mg,g)}^G\times P_{(t=1,mg,g)}^G)\\
+\sum_{mg \in MG}[\sum_{c\in BAT}(c_{(t=1,mg,c)}^{ch}\times P_{(t=1,mg,c)}^{ch}-c_{(t=1,mg,c)}^{dch}\times P_{(t=1,mg,c)}^{dch})\\
+
\begin{bmatrix}
\lambda_{1}^{t} & \lambda_{2}^{t} & \dots & \lambda_{m(m-1)}^{t}
\end{bmatrix}
.
\begin{bmatrix}
    P_{mg=1,t}^{buy,MG1-MG2}-P_{mg=2,t}^{sell,MG2-MG1} \\
    P_{mg=1,t}^{buy,MG1-MG3}-P_{mg=3,t}^{sell,MG3-MG1} \\
    \vdots \\
    P_{mg=m,t}^{buy,MGm-MGn}-P_{mg=n,t}^{sell,MGn-MGm} \\
    P_{mg=n,t}^{buy,MGn-MGm}-P_{mg=m,t}^{sell,MGm-MGn}
\end{bmatrix}
\end{split}
\end{equation}

\begin{equation}
\label{tr02}\footnotesize
\begin{split}
&L(P,\lambda)=\sum_{mg \in MG}[\sum_{g\in DG}(c_{(t=1,mg,g)}^G\times P_{(t=1,mg,g)}^G)\\
&+\sum_{mg \in MG}[\sum_{c\in BAT}(c_{(t=1,mg,c)}^{ch}\times P_{(t=1,mg,c)}^{ch}-c_{(t=1,mg,c)}^{dch}\times P_{(t=1,mg,c)}^{dch})\\
&+\lambda_{1}^{t}(P_{(mg=1,t)}^{buy,MG1-MG2}-P_{(mg=2,t)}^{sell,MG2-MG1})\\
&+\lambda_{2}^{t}(P_{(mg=2,t)}^{buy,MG2-MG1}-P_{(mg=1,t)}^{sell,MG1-MG2})\\
&+\lambda_{3}^{t}(P_{(mg=2,t)}^{buy,MG2-MG3}-P_{(mg=3,t)}^{sell,MG3-MG2})\\
&+\lambda_{4}^{t}(P_{(mg=3,t)}^{buy,MG3-MG2}-P_{(mg=2,t)}^{sell,MG2-MG3})\\
&+\lambda_{5}^{t}(P_{(mg=3,t)}^{buy,MG3-MG4}-P_{(mg=4,t)}^{sell,MG4-MG3})\\
&+\lambda_{6}^{t}(P_{(mg=4,t)}^{buy,MG4-MG3}-P_{(mg=3,t)}^{sell,MG3-MG4})
\end{split}
\end{equation}

\begin{equation}
\label{tr03}\footnotesize
\begin{split}
& \underset{mg=1}{min} [\sum_{g\in DG}(c_{(t,mg=1,g)}^G\times P_{(t,mg=1,g)}^G)\\
&+\sum_{c\in BAT}(c_{(t,mg=1,c)}^{ch}\times P_{(t,mg=1,c)}^{ch}-c_{(t,mg=1,c)}^{dch}\times P_{(t,mg=1,c)}^{dch})\\
&+\lambda_{1}^{t}(P_{(mg=1,t)}^{buy,MG1-MG2})-\lambda_{2}^{t}(P_{(mg=1,t)}^{sell,MG1-MG2})]
\end{split}
\end{equation}

\begin{equation}
\label{tr04}\footnotesize
\begin{split}
& \underset{mg=2}{min} [\sum_{g\in DG}(c_{(t,mg=2,g)}^G\times P_{(t,mg=2,g)}^G)\\
&+\sum_{c\in BAT}(c_{(t,mg=2,c)}^{ch}\times P_{(t,mg=2,c)}^{ch}-c_{(t,mg=2,c)}^{dch}\times P_{(t,mg=2,c)}^{dch})\\
&+\lambda_{2}^{t}(P_{(mg=2,t)}^{buy,MG2-MG1})+\lambda_{3}^{t}(P_{(mg=2,t)}^{buy,MG2-MG3})\\
&-\lambda_{1}^{t}(P_{(mg=2,t)}^{sell,MG2-MG1})-\lambda_{4}^{t}(P_{(mg=2,t)}^{sell,MG2-MG3})]
\end{split}
\end{equation}

\begin{equation}
\label{tr05}\footnotesize
\begin{split}
& \underset{mg=3}{min} [\sum_{g\in DG}(c_{(t,mg=3,g)}^G\times P_{(t,mg=3,g)}^G)\\
&+\sum_{c\in BAT}(c_{(t,mg=3,c)}^{ch}\times P_{(t,mg=3,c)}^{ch}-c_{(t,mg=3,c)}^{dch}\times P_{(t,mg=3,c)}^{dch})\\
&+\lambda_{4}^{t}(P_{(mg=3,t)}^{buy,MG3-MG2})+\lambda_{5}^{t}(P_{(mg=3,t)}^{buy,MG3-MG4})\\
&-\lambda_{3}^{t}(P_{(mg=3,t)}^{sell,MG3-MG2})-\lambda_{6}^{t}(P_{(mg=3,t)}^{sell,MG3-MG4})]
\end{split}
\end{equation}

\begin{equation}
\label{tr06}\footnotesize
\begin{split}
& \underset{mg=4}{min} [\sum_{g\in DG}(c_{(t,mg=4,g)}^G\times P_{(t,mg=4,g)}^G)\\
&+\sum_{c\in BAT}(c_{(t,mg=4,c)}^{ch}\times P_{(t,mg=4,c)}^{ch}-c_{(t,mg=4,c)}^{dch}\times P_{(t,mg=4,c)}^{dch})\\
&+\lambda_{6}^{t}(P_{(mg=4,t)}^{buy,MG4-MG3})-\lambda_{5}^{t}(P_{(mg=4,t)}^{sell,MG4-MG3})]
\end{split}
\end{equation}

Therefore, in a network with $m$ MG, there are $m$ sub-problem. Besides, each sub-problem should include $2(m-1)$ multipliers, which means that each microgrid can connected to other $(m-1)$ MG to purchase or sell power. So, we will have $(m-1)$ multipliers for purchasing power and $(m-1)$ multipliers for selling power.

\begin{equation}
\label{eq38}\footnotesize
\begin{split}
\underset{MG_{m}}{min}\{\sum_{g\in DG}(c_{(t,mg=m,g)}^G\times P_{(t,mg=m,g)}^G)\\
+[\sum_{c\in BAT}(c_{(t,mg=m,c)}^{ch}\times P_{(t,mg=m,c)}^{ch}\\
-c_{(t,mg=m,c)}^{dch}\times P_{(t,mg=m,c)}^{dch})]\\
+[\lambda^{(t)}]^{T}.[(P_{mg=m,t}^{buy/sell,MG_{m}-MG_{n}})]\}
\end{split}
\end{equation}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.50\textwidth]{images/new02}
% 	\caption{\small Distributed and Asynchronous implementation of Surrogate Lagrangian Relaxation}
% 	\label{fignew02}\vspace{-10px}
% \end{figure}


\subsection{Linearization of the droop controlled equations}\label{Section:04:02}
For droop buses, we have (\ref{eq033}) and (\ref{q034}), which make the problem nonlinear. In (\ref{eq033}), which is the real power balance in droop control buses, $m_{p}$ is a discrete value, while $f_{mg}$ is the continuous variable. Let's assume that $k_{p}=\frac{1}{m_{p}}$. Therefore, the product of the discrete variable $k_{p}$ and continuous variable $f_{mg}$ ($w=k_{p}.f_{mg}$) is nonlinear. Now, we can use the linearization rule discussed in previous subsection to convert the problem to a linear one.
\begin{equation}
\label{eq34}\footnotesize
w_{j}=k_{p,j}.f_{mg}, \quad \forall j\in J
\end{equation}

Now, we can replace (\ref{eq34}) by inequality constraints, similar to (\ref{eq31})-(\ref{eq33}), to get rid of non-linearity. Therefore, we can rewrite (\ref{eq33}) as below:
\begin{equation}
\label{eq0035}\footnotesize
z_{j}=\sum_{i=0}^{X}i.w_{ij}.f_{mg}, \quad \forall j\in J
\end{equation}

Also, the inequality constraints mentioned in (\ref{eq27})-(\ref{eq30}) should be considered for each $j$. Finally, the non-linear equality constraint (\ref{eq033}) can be rewrite as following subject to constraints (\ref{eq27})-(\ref{eq32}) and (\ref{eq35}):
\begin{equation}
\label{eq36}\footnotesize
\begin{split}
P_{i,j}^{f,t}=\sum_{(k:(j,k))\in N}P_{j,k}^{f,t}+ PL^{i}_{mg,t}\\
-(P^{buy}_{mg,t}-P^{sell}_{mg,t})-(P^{dch}_{mg,t}-P^{ch}_{mg,t}),\\ \quad\forall t\in T, i,j,k\in N
\end{split}
\end{equation}
%\begin{equation}
%\label{eq36}\footnotesize
%\begin{split}
%PL^{m}_{mg,t}-(P^{buy}_{mg,t}-P^{sell}_{mg,t})-\\
%(P^{dch}_{mg,t}-P^{ch}_{mg,t})=P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- %\sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, %m,n\in M
%\end{split}
%\end{equation}

Similarly, for the reactive power balance in droop control buses, $m_{q}$ is a discrete value, while $|V|_{mg}$ is the continuous variable. Let's assume that $k_{q}=\frac{1}{m_{q}}$. So, the nonlinear term is as follows:
\begin{equation}
\label{eq37}\footnotesize
w_{j}=k_{q,j}.|V|_{mg}, \quad \forall j\in J
\end{equation}

Now, we can replace (\ref{eq37}) by inequality constraints, similar to (\ref{eq31})-(\ref{eq33}), to get rid of non-linearity. Therefore, we can rewrite (\ref{eq33}) as below:
\begin{equation}
\label{eq0038}\footnotesize
z_{j}=\sum_{i=0}^{X}i.w_{ij}.|V|_{mg}, \quad \forall j\in J
\end{equation}

Finally, the non-linear equality constraint (\ref{q034}) can be rewrite as following subject to constraints (\ref{eq27})-(\ref{eq32}) and (\ref{eq0038}):
\begin{equation}
\label{eq0039}\footnotesize
\begin{split}
Q_{i,j}^{f,t}=\sum_{(k:(j,k))\in N}Q_{j,k}^{f,t}+ QL^{m}_{mg,t}, \quad\forall t\in T, i,j,k\in N
\end{split}
\end{equation}
%\begin{equation}
%\label{eq39}\footnotesize
%\begin{split}
%QL^{m}_{mg,t}=Q_{nm}^{flow,t}-x_{nm}\times l_{nm}^t- \sum_{\kappa \in (m,\kappa)}(Q_{m\kappa}^{flow,t}),\\ \quad\forall t\in T
%\end{split}
%\end{equation}



%%%%% Nomenclature

%\section{Nomenclature}\label{sez:4\part{title}}
\vspace{-5px}
%\vspace{8px}
	\mbox{}
	%\scriptsize{
%		\footnotesize {
	\setlength{\nomlabelwidth}{2cm}
	\setlength{\nomitemsep}{-\parsep}
	    \nomenclature[A,01]{$t$}{Index of time}
	    \nomenclature[A,02]{$r$}{Index for iteration number of DA-SLR}
	    \nomenclature[A,03]{$m, w$}{Indices of microgrids}
	    \nomenclature[A,04]{$c$}{Index of battery}
	    \nomenclature[A,05]{$n,k$}{Indices of bus}
	    
	    
		\nomenclature[B,01]{$\alpha^{g}$}{Power generation price of dispatchable DGs}
		\nomenclature[B,02]{$\alpha_{ch}^{BAT}$}{Charging price of the battery}
		\nomenclature[B,03]{$\alpha_{dch}^{BAT}$}{Discharging price of the battery}
		\nomenclature[B,04]{$f_{ref}$}{Nominal frequency [Hz]}
		\nomenclature[B,05]{$V_{ref}$}{Nominal voltage magnitude [v]}
		\nomenclature[B,06]{$V_{0}$}{The bus voltage magnitude of point of common coupling in an MG [v]}
		\nomenclature[B,07]{$r_{n,k}$}{Distribution line resistance between nodes $n$ and $k$}
		\nomenclature[B,08]{$x_{n,k}$}{Distribution line reactance between nodes $n$ and $k$}
		\nomenclature[B,09]{$\zeta_{IL}$}{Interrupted power price}
		\nomenclature[B,10]{$s_{n}^{g}$}{Connection indicator of a generator to node $n$}
		\nomenclature[B,11]{$s_{n}^{BAT}$}{Connection indicator of a battery to node $n$}
		\nomenclature[B,12]{$s_{n-m}^{Tran}$}{Connection indicator of node $n$ to a node in neighbour MG $m$}
		\nomenclature[B,13]{$P_{t}^{g,WT}$}{Real power generation of a wind turbine at time $t$ [kW]}
		\nomenclature[B,14]{$P_{t}^{g,PV}$}{Real power generation of a PV at time $t$ [kW]}
		\nomenclature[B,15]{$Q_{t}^{g,WT}$}{Reactive power generation of a wind turbine at time $t$ [kvar]}
		\nomenclature[B,16]{$Q_{t}^{g,PV}$}{Reactive power generation of a PV at time $t$ [kvar]}
		
		\nomenclature[c,01]{$P^{g,MT}$}{Generated power by MT [kW]}
		\nomenclature[c,02]{$P^{g,FC}$}{Generated power by FC [kW]}
		\nomenclature[c,03]{$P^{g,CHP}$}{Generated power by CHP [kW]}
		\nomenclature[c,04]{$P^{BAT,ch}$}{Charging power of battery [kW]}
		\nomenclature[c,05]{$P^{BAT,dch}$}{Discharging power of battery [kW]}
		\nomenclature[c,06]{$Q^{g,DG}$}{Generated reactive power of a DG [kW]}
		\nomenclature[c,07]{$f$}{Frequency [Hz]}
		\nomenclature[c,08]{$V$}{Voltage magnitude [v]}
		\nomenclature[c,09]{$m_{p}$}{f-P related droop coefficient}
		\nomenclature[c,10]{$m_{q}$}{V-Q related droop coefficient}
		\nomenclature[c,11]{$P_{(t,n-k)}^{flow}$}{Real power flow between nodes $n$ and $k$ at hour $t$}
		\nomenclature[c,12]{$Q_{(t,n-k)}^{flow}$}{Reactive power flow between nodes $n$ and $k$ at hour $t$}
		\nomenclature[c,13]{$P_{(t,k)}^{L}$}{Real load power in node $k$ at hour $t$}
		\nomenclature[c,14]{$Q_{(t,k)}^{L}$}{Reactive load power in node $k$ at hour $t$}
		\nomenclature[c,15]{$C_{g}$}{Power generation cost [\$/kWh]}
		\nomenclature[c,16]{$C_{ch}$}{Battery charging cost [\$/kWh]}
		\nomenclature[c,17]{$C_{dch}$}{Battery discharging cost [\$/kWh]}
		\nomenclature[c,18]{$P^{IL}$}{Real power interruption [kW]}
		\nomenclature[c,19]{$Q^{IL}$}{Reactive power interruption [kvar]}
		\nomenclature[c,20]{$u^{g}$}{Commitment status of a generator}
		\nomenclature[c,21]{$u^{buy}$}{Status of purchasing power buy MG $m$}
		\nomenclature[c,22]{$P_{(t,m)}^{buy}$}{Real purchased power by MG $m$ at hour $t$ [kW]}
		\nomenclature[c,23]{$P_{(t,m)}^{sell}$}{Real sold power by MG $m$ at hour $t$ [kW]}
		\nomenclature[c,24]{$Q_{(t,m)}^{buy}$}{Reactive purchased power by MG $m$ at hour $t$ [kvar]}
		\nomenclature[c,25]{$Q_{(t,m)}^{sell}$}{Reactive sold power by MG $m$ at hour $t$ [kvar]}
		\nomenclature[c,26]{$u^{ch}$}{Status of charging power by a battery}
		\nomenclature[c,27]{$\lambda^{\alpha}$}{$\alpha th$ Lagrange multiplier}
		
		
		\nomenclature[D,01]{$MG$}{Microgrid}
		\nomenclature[D,02]{$DER$}{Distributed energy resource}
		\nomenclature[D,03]{$DNO$}{Distribution network operator}
		\nomenclature[D,04]{$WT$}{Wind turbine}
		\nomenclature[D,05]{$PV$}{Photovoltaic panel}
		
	
	\printnomenclature
%}\vspace{-5px} 



\section{Problem formulation}\label{Section:02}
\subsection{Objective function}\label{Subsection:new:01}
The objective function of the networked MGs is described as following in the centralized mode.
\begin{equation}
\label{eq01}\footnotesize
\begin{split}
OF=& \sum_{t \in T}\sum_{m \in MG}[\sum_{i\in I}(\alpha_{MT}\times P_{(t,m,i)}^{g,MT}+\alpha_{CHP}\times P_{(t,m,i)}^{g,CHP}\\
& +\alpha_{FC}\times P_{(t,m,i)}^{g,FC})+\sum_{b \in B}(\beta_{dch}\times P_{(t,m,b)}^{dch}-\beta_{ch}\times P_{(t,m,b)}^{ch})\\
& +\zeta_{IL}\times P_{(t,m)}^{IL}+\zeta_{IL}\times Q_{(t,m)}^{IL}]
\end{split}
\end{equation}

where, $\alpha_{MT}$, $\alpha_{CHP}$ and $\alpha_{FC}$ are generation price coefficients of MT, CHP and FC. $P_{(t,m,i)}^{g,MT}$, $P_{(t,m,i)}^{g,CHP}$ and $P_{(t,m,i)}^{g,FC}$ are the generated power of MT, CHP and FC in $mth$ microgrid at hour $t$. $\beta_{dch}$ and $\beta_{ch}$ are discharging and charging price coefficients of batteries. $P_{(t,m,b)}^{dch}$ and $P_{(t,m,b)}^{ch}$ are discharging and charging powers of batteries in $mth$ MG at hour $t$. Also, $\zeta_{IL}$ is the price of interrupted power. $P_{(t,m)}^{IL}$ and $Q_{(t,m)}^{IL}$ are the active and reactive interrupted powers in $mth$ MG at hour $t$.

\subsection{Constraints}\label{Subsection:new:02}
The MGs should consider a set of financial and technical constraints which are described in the following.
\subsubsection{Operational limits}\label{Subsubsection:02:03:01}

In (\ref{eq12}) and (\ref{eq12q}), the active and reactive generation range of DGs including MT, CHP and FC can be seen. It should be mentioned that MT, CHP and FC are utilized to generate active power, while only MT and CHP units are considered for reactive power generation.
\begin{equation}
\label{eq12}\footnotesize
u_{g,DG}^{t}.P_{min,DG}^{t}\leq P_{g,DG}^{t}\leq  u_{g,DG}^{t}.P_{max,DG}^{t}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq12q}\footnotesize
u_{g,DG}^{t}.Q_{min,DG}^{t}\leq Q_{g,DG}^{t}\leq  u_{g,DG}^{t}.Q_{max,DG}^{t}, \quad \forall t\in T
\end{equation}

where, $u_{g,DG}$ is a binary variable to describe the commitment status of a DG unit. $P_{g,DG}^{t}$ and $Q_{g,DG}^{t}$ are the active and reactive power generation of a DG at hour $t$.

The limits dealing with purchased and sold powers are described as (\ref{eq13}) and (\ref{eq14}) for active powers. Also, (\ref{eq13q}) and (\ref{eq14q}) are used for reactive power interaction. It should be mentioned that each MG cannot purchase and sell power at the same hour. To model this, a binary variable $u_{(t,m)}^{buy}$ is used to prevent purchasing and selling power at the same time.
\begin{equation}
\label{eq13}\footnotesize
0\leq P_{(t,m)}^{buy}\leq  u_{(t,m)}^{buy}.P_{max}^{buy}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq14}\footnotesize
0\leq P_{(t,m)}^{sell}\leq  (1-u_{(t,m)}^{buy}).P_{max}^{sell}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq13q}\footnotesize
0\leq Q_{(t,m)}^{buy}\leq  u_{(t,m)}^{buy}.Q_{max}^{buy}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq14q}\footnotesize
0\leq Q_{(t,m)}^{sell}\leq  (1-u_{(t,m)}^{buy}).Q_{max}^{sell}, \quad \forall t\in T
\end{equation}

where, $u_{(t,m)}^{buy}$ is a binary variable of the power interaction status. $P_{(t,m)}^{buy}$ and $P_{(t,m)}^{sell}$ are active purchased and sold powers of $mth$ MG at hour $t$, while $Q_{(t,m)}^{buy}$ and $Q_{(t,m)}^{sell}$ are dealing with reactive power interaction.

Also, in (\ref{eq15}) and (\ref{eq16}), the constraints of charging and discharging powers are described. It is noted that a binary variable, $u_{(t,m)}^{ch}$ is used to prevent charging and discharging power at the same hour.
\begin{equation}
\label{eq15}\footnotesize
0\leq P_{(t,m)}^{ch}\leq  u_{(t,m)}^{ch}.P_{max}^{ch}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq16}\footnotesize
0\leq P_{(t,m)}^{dch}\leq  (1-u_{(t,m)}^{ch}).P_{max}^{dch}, \quad \forall t\in T
\end{equation}

where, $u_{(t,m)}^{ch}$ is a binary variable of charging status of the batteries. $P_{(t,m)}^{ch}$ and $P_{max}^{dch}$ are charging and discharging powers of $mth$ MG at hour $t$.

Additionally, the active and reactive power flow in the distribution lines are in a technical range as follows:
\begin{equation}
\label{eq17new}\footnotesize
P_{(min)}^{flow}\leq P_{(t,n-k)}^{flow}\leq  P_{(max)}^{flow}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq18new}\footnotesize
Q_{(min)}^{flow}\leq Q_{(t,n-k)}^{flow}\leq  Q_{(max)}^{flow}, \quad \forall t\in T
\end{equation}

where, $P_{(t,n-k)}^{flow}$ and $Q_{(t,n-k)}^{flow}$ are active and reactive power flow between $nth$ node and $kth$ node at hour $t$.

Also, the inequality constraints dealing with  active and reactive powers shedding are defined as follows:
\begin{equation}
\label{eq19new}\footnotesize
0\leq P_{(t,n)}^{int}\leq  P_{(max)}^{int}, \quad \forall t\in T
\end{equation}
\begin{equation}
\label{eq20new}\footnotesize
0\leq Q_{(t,n)}^{int}\leq  Q_{(max)}^{int}, \quad \forall t\in T
\end{equation}

where, $P_{(t,n)}^{int}$ and $Q_{(t,n)}^{int}$ are active and reactive interrupted powers in $nth$ node at hour $t$.

The limit for voltage magnitude for each node can be described as follows:
\begin{equation}
\label{eq21new}\footnotesize
|V_{min}|\leq |V_{(t,n)}|\leq  |V_{max}|, \quad \forall t\in T
\end{equation}

where, $|V_{(t,n)}|$ is the voltage magnitude of $nth$ node at hour $t$.
\subsubsection{Power balance constraints}\label{Subsubsection:02:03:02}

According to the droop control features, the frequency and voltage of each microgrid depend on the active and reactive power deviations. P–f and Q–V droop based control can be described as follows:
\begin{equation}
\label{eq22new}\footnotesize
\begin{split}
f=f^{ref}-m_{p}(P_{g,DG}-P_{g,DG}^{ref})
\end{split}
\end{equation}
\begin{equation}
\label{eq23new}\footnotesize
\begin{split}
|V|=|V^{ref}|-m_{q}(Q_{g,DG}-Q_{g,DG}^{ref})
\end{split}
\end{equation}

where, $f$ as a continuous variable is the frequency. $f^{ref}$ is the reference frequency. $m_{p}$ and $m_{q}$ are droop control coefficients. $P_{g,DG}^{ref}$ and $Q_{g,DG}^{ref}$ are reference values for active and reactive powers of DGs. $|V^{ref}|$ is the reference value of the voltage magnitude. It should be mentioned that the range of frequency is considered as follows:
\begin{equation}
\label{eqfnew}\footnotesize
\begin{split}
59.5\leq f_{t}\leq  60.5, \quad \forall t\in T
\end{split}
\end{equation}

However, the equations dealing with (\ref{eq22new}) and (\ref{eq23new}) are non-linear, which should be linearized first.

Suppose the expression $z=A\times x$, where $A$ is a continuous variable and $x$ is a binary variable. If $A$ has bounds $[\bar{A},\underaccent{\bar}{A}]$,  then the form of the linearized inequalities are as following for expression $z$:
\begin{equation}
\label{eq27}\footnotesize
min\{0,\underaccent{\bar}{A}\}\leq z\leq \bar{A}
\end{equation}
\begin{equation}
\label{eq28}\footnotesize
\underaccent{\bar}{A}x\leq z\leq \bar{A}x
\end{equation}
\begin{equation}
\label{eq29n}\footnotesize
A-(1-x)\bar{A}\leq z\leq A-(1-x)\underaccent{\bar}{A}
\end{equation}
\begin{equation}
\label{eq30n}\footnotesize
z\leq A+(1-x)\bar{A}
\end{equation}

If $x=0$ then $z$ has to be zero as well. See how this is automatically enforced by inequality (\ref{eq28}). Now, if $x=1$ then $z$ has to be equal to $A$. See how this is also enforced by the inequality (\ref{eq29n}). The others are there to ensure everything work.

However, in the proposed model, $x$ is not a binary variable but a discrete variable (integer non-negative variable). If $x_{j}$ can be bounded by positive integer $X$, so that $x_{j}\in \{0,1,...,X\}$, we can introduce binary variables $w_{0},w_{1},...,w_{X}$ and add the following constraints:
\begin{equation}
\label{eq31}\footnotesize
\sum_{i=0}^{X}w_{ij}=1, \quad \forall j\in J
\end{equation}
\begin{equation}
\label{eq32}\footnotesize
x_{j}=\sum_{i=0}^{X}i.w_{ij}, \quad \forall j\in J
\end{equation}

Therefore:
\begin{equation}
\label{eq33}\footnotesize
z_{j}=\sum_{i=0}^{X}i.w_{ij}.A, \quad \forall j\in J
\end{equation}

Now, we can linearize each of the products of $w_{ij}.A$ based on inequalities (\ref{eq27})-(\ref{eq30n}).

For droop buses, we have (\ref{eq22new}) and (\ref{eq23new}), which make the problem nonlinear. In (\ref{eq22new}), $m_{p}$ is a discrete value, while $f$ is the continuous variable. Let's assume that $k_{p}=\frac{1}{m_{p}}$. Therefore, the product of the discrete variable $k_{p}$ and continuous variable $f$ ($w=k_{p}.f$) is nonlinear. Now, we can use the linearization rule discussed in previous subsection to convert the problem to a linear one.
\begin{equation}
\label{eq34}\footnotesize
w_{j}=k_{p,j}.f, \quad \forall j\in J
\end{equation}

Now, we can replace (\ref{eq34}) by inequality constraints, similar to (\ref{eq31})-(\ref{eq33}), to get rid of non-linearity. Therefore, we can rewrite (\ref{eq33}) as below:
\begin{equation}
\label{eq35}\footnotesize
z_{j}=\sum_{i=0}^{X}i.w_{ij}.f, \quad \forall j\in J
\end{equation}

%\begin{equation}
%\label{eq36}\footnotesize
%\begin{split}
%PL^{m}_{mg,t}-(P^{buy}_{mg,t}-P^{sell}_{mg,t})-\\
%(P^{dch}_{mg,t}-P^{ch}_{mg,t})=P_{nm}^{flow,t}-r_{nm}\times l_{nm}^t- %\sum_{\kappa \in (m,\kappa)}(P_{m\kappa}^{flow,t}),\\ \quad\forall t\in T, %m,n\in M
%\end{split}
%\end{equation}

Similarly, for the reactive power balance in droop control buses, $m_{q}$ is a discrete value, while $|V_{n}|$ is the continuous variable. Let's assume that $k_{q}=\frac{1}{m_{q}}$. So, the nonlinear term is as follows:
\begin{equation}
\label{eq37}\footnotesize
w_{j}=k_{q,j}.|V_{n}|, \quad \forall j\in J
\end{equation}

Now, we can replace (\ref{eq37}) by inequality constraints, similar to (\ref{eq31})-(\ref{eq33}), to get rid of non-linearity. Therefore, we can rewrite (\ref{eq33}) as below:
\begin{equation}
\label{eq38}\footnotesize
z_{j}=\sum_{i=0}^{X}i.w_{ij}.|V_{n}|, \quad \forall j\in J
\end{equation}

In this paper, linearized DistFlow model is utilized, which is an exact approximation of AC power flow \cite{51wang2015coordinated}. The linearized DistFlow equations are listed as follows:
\begin{equation}
\label{r06}\footnotesize
\begin{split}
P_{(t,n-k)}^{flow}=\sum_{(\kappa:(k,\kappa))\in N}P_{(t,k-\kappa)}^{flow}-(P_{(t,k)}^{g}-P_{(t,k)}^{L}), \\
\quad\forall t\in T,\ n,k,\kappa\in N
\end{split}
\end{equation}
\begin{equation}
\label{r07}\footnotesize
\begin{split}
Q_{(t,n-k)}^{flow}=\sum_{(\kappa:(k,\kappa))\in N}P_{(t,k-\kappa)}^{flow}-(Q_{(t,k)}^{g}-Q_{(t,k)}^{L}), \\
\quad\forall t\in T,\ n,k,\kappa\in N
\end{split}
\end{equation}
\begin{equation}
\label{r08}\footnotesize
\begin{split}
|V_{(n,t)}|=|V_{(k,t)}|-\frac{r_{n,k}\times P_{(t,n-k)}^{flow}+x_{n,k}\times Q_{(t,n-k)}^{flow}}{|V_{0}|} \\
\quad\forall t\in T,\ n,k\in N
\end{split}
\end{equation}
where, $P_{(t,n-k)}^{flow}$ and $Q_{(t,n-k)}^{flow}$ are real and reactive power flow from node $n$ to node $k$ at time $t$, respectively. $P_{(t,k)}^{g}$, and $Q_{(t,k)}^{g}$ are real and reactive power generation of node $k$ at time $t$, respectively. Also, $P_{(t,k)}^{L}$, and $Q_{(t,k)}^{L}$ are real and reactive power consumption of node $k$, respectively. $V_{0}$ is the bus voltage of the point of common coupling (PCC) in the microgrid. $r_{n,k}$ and $x_{n,k}$ are resistance and reactance of the line between node $n$ and $k$.

The active and reactive power balance constraints in bus $n$ of each MG at hour $t$ could be written as follows: \cite{8207635}:
\begin{equation}
\label{eq033p}\footnotesize
\begin{split}
&(s_{n}^{MT}.P_{(n,t)}^{g,MT}+s_{n}^{CHP}.P_{(n,t)}^{g,CHP}+s_{n}^{FC}.P_{(n,t)}^{g,FC}+s_{n}^{WT}.P_{(n,t)}^{g,WT}+s_{n}^{PV}.P_{(n,t)}^{g,PV})\\
&+(s_{n}^{BAT}.P_{(n,t)}^{dch}-s_{n}^{BAT}.P_{(n,t)}^{ch})+\sum_{(k:(n,k))\in N}P_{(t,n-k)}^{flow}+P_{(n,t)}^{IL}\\
&+(\sum_{m \in MG}(s_{n-m}^{Tran}.P_{(t,n-m)}^{buy}-s_{n-m}^{Tran}.P_{(t,n-m)}^{sell}))+\frac{1}{m_{p}}(f_{(n)}^{ref}-f_{(t,n)}^{ref})\\
&=P_{(t,n)}^{L},\quad\forall t\in T, n,k\in N
\end{split}
\end{equation}
\begin{equation}
\label{eq033q}\footnotesize
\begin{split}
&(s_{n}^{MT}.Q_{(n,t)}^{g,MT}+s_{n}^{CHP}.Q_{(n,t)}^{g,CHP}+s_{n}^{WT}.Q_{(n,t)}^{g,WT}+s_{n}^{PV}.Q_{(n,t)}^{g,PV})\\
&+\sum_{(k:(n,k))\in N}Q_{(t,n-k)}^{flow}+Q_{(n,t)}^{IL}+(\sum_{m \in MG}(s_{n-m}^{Tran}.Q_{(t,n-m)}^{buy}-s_{n-m}^{Tran}.Q_{(t,n-m)}^{sell}))\\
&+\frac{1}{m_{q}}(|V_{n}^{ref}|-|V_{(n,t)}|)=Q_{(t,n)}^{L}, \quad\forall t\in T, n,k\in N
\end{split}
\end{equation}

where, $s_{n}$ is the commitment status of a variable.







